Frequency-noise-insensitive universal control of Kerr-cat qubits

We theoretically study the influence of frequency uncertainties on the operation of a Kerr-cat qubit. As the mean photon number increases, Kerr-cat qubits provide an increasing level of protection against phase errors induced by unknown frequency shifts during idling and X rotations. However, realizing rotations about the other principal axes (e.g., Y and Z axes) while preserving robustness is nontrivial. To address this challenge, we propose a universal set of gate schemes which circumvents the tradeoff between protection and controllability in Kerr-cat qubits and retains robustness to unknown frequency shifts to at least first order. Assuming an effective Kerr oscillator model, we theoretically and numerically analyze the robustness of elementary gates on Kerr-cat qubits, with special focus on gates along nontrivial rotation axes. An appealing application of this qubit design would include tunable superconducting platforms, where the induced protection against frequency noise would allow for a more flexible choice of operating point and thus the potential mitigation of the impact of spurious two-level systems.

==> main_notes.tex <==
\clearpage
\begin{itemize}
    \item rather short, succinct paper (PRL length)
    \item initial motivation
    \item describing the gates and robustness systematically
    \item 2q gate easy bc analogous to 1q X; compare analytics of X to those of XX, exponential suppression of relevant error matrix element
    \item brief section why Y is challenging (mention DRAG maybe in SI), and then Z in more detail in longer section [view Y as motivation for design of better gate -> Z]
    \item full cosine? -> (before) discussion section, maybe even only qualitatively, couple paragraphs
    \item mention in/before discussion (especially in light of Z gate): detuned KC as base qubit / conclusion
    \item in this paper the base qubit is the non-detuned qubit
    \item time.dependent detuning as brief addition together in dicussion with the phase space trajectories of the different Z gates (optimal for static vs better for dynamic case). Error rate as function of power spectral density can be mentioned but derived in the appendix. Maybe show these two trajectories and plot the relevant function that shows w=0 suppression for static case and low weight for dynamic case around w=0.
\end{itemize}
Next steps:
\begin{itemize}
    \item literature search!!
    \item put together figures and key points to get first impression of overall picture ("shell")
\end{itemize}

Plots:
\begin{itemize}
    \item cartoon figure where the initial motivation (TLSs) is highlighted, could be $\omega(\phi)$ plot, and then come back to that theme throughout
    \item Matrix elements
    \item Robustness figures for X, Y, Z
    \item phase space pictures Z gate
    \item power spectral density in conjunction
\end{itemize}
